Quantifying and Defending against Privacy Threats on Federated Knowledge Graph Embedding

Knowledge Graph Embedding (KGE) is a fundamental technique that extracts expressive representation from knowledge graph (KG) to facilitate diverse downstream tasks. The emerging federated KGE (FKGE) collaboratively trains from distributed KGs held among clients while avoiding exchanging clients' sensitive raw KGs, which can still suffer from privacy threats as evidenced in other federated model trainings (e.g., neural networks). However, quantifying and defending against such privacy threats remain unexplored for FKGE which possesses unique properties not shared by previously studied models. In this paper, we conduct the first holistic study of the privacy threat on FKGE from both attack and defense perspectives. For the attack, we quantify the privacy threat by proposing three new inference attacks, which reveal substantial privacy risk by successfully inferring the existence of the KG triple from victim clients. For the defense, we propose DP-Flames, a novel differentially private FKGE with private selection, which offers a better privacy-utility tradeoff by exploiting the entity-binding sparse gradient property of FKGE and comes with a tight privacy accountant by incorporating the state-of-the-art private selection technique. We further propose an adaptive privacy budget allocation policy to dynamically adjust defense magnitude across the training procedure. Comprehensive evaluations demonstrate that the proposed defense can successfully mitigate the privacy threat by effectively reducing the success rate of inference attacks from $83.1\%$ to $59.4\%$ on average with only a modest utility decrease.

==> attack_copy.tex <==
\section{Attack} \label{sec: attack}
In this section, we first propose a threat model to characterize background knowledge of adversaries with different identities.
Then, we formally define our membership inference attacks and explain their attack mechanisms in detail.
\subsection{Threat Model} \label{subsection: threat model}
\partitle{Adversary's Goal} 
The adversary's goal is to determine whether a triple $(h,r,t)$ is in the training dataset of the victim clients contributing to the federated learning.
% have a KGE model.
Triples are usually viewed as sensitive private information of the knowledge graph owner.
When a triple represents user's sensitive behavior, inferring the triple leads to a severe privacy threat.
For example, the account behavior of bank users is related to their business activities, and adversaries can infer relevant triples to obtain illegal business benefits.
Although FKGE communicates only the intermediate embedding of clients and avoids the raw triples to be exchanged directly, adversaries can still attempt to infer the existence of the victim triples by  exploiting information carried by the communicated embeddings.

\partitle{Adversary's Background Knowledge}
In this paper, for a victim knowledge graph $\mathcal{G}_v$,  we consider that adversaries can be a malicious client $\mathcal{G}_a$ or server $S_a$.
When the adversary is a client, besides its own data, $\mathcal{G}_a$ can also obtain entity embedding matrix from the server.
From the perspective of the malicious server, $S_a$ has the victim model's entity set $\mathcal{E}_v$ and the entity embedding matrix $\bf{E}_v$ uploaded by the victim model.
In addition, due to the characteristics of federated learning, the KGE training algorithm and score function used by the victim model is public information.
Note that inferring sensitive information of FKGE graph is more challenging than previous work where adversaries have entire updates or prediction vectors.
\subsection{Attack Taxonomy}
We propose three inference attacks that can infer triples of the target knowledge graph holder, including the passive transfer inference attack ($\mathcal{F}_{pt}$), the active transfer inference attack ($\mathcal{F}_{at}$) and the relation inference attack ($\mathcal{F}_{re}$).
Different attack methods vary in identities, capabilities, and auxiliary information. The attacks are summarized in Table \ref{table: attack}.

\partitle{Identity}
As mentioned in Section \ref{subsection: threat model}, both clients and servers in FKGE have the ability to be adversaries. Our proposed attacks method focuse on unilateral attack scenarios rather than multi-party collusion, which is more challenging.

\partitle{Capability}
In federated learning, an active adversary not only observes the information, but can also modify it. Our attack methods are divided into passive attacks and active attacks, which have the ability to observe or modify information, respectively. 

\partitle{Auxiliary Dataset}
To infer complete triples, we assume the server has an auxiliary dataset $\mathcal{D}_{aux}$ that comes from practical inference on the victim knowledge graph. For example, we could know the knowledge of $(patient, have, disease)$ when a knowledge graph belongs to a hospital.

\begin{table}[h]
    \caption{An overview of the different types of attacks}
    \label{table: attack}
    \begin{tabular}{cccc}
      \toprule
      Attack type & Identity & Capability & Auxiliary dataset\\
      \midrule
      $\mathcal{F}_{pt}$ & client & observation & -\\
      $\mathcal{F}_{at}$ & client & modification & -\\
      $\mathcal{F}_{re}$ & server & observation & \checkmark\\
      \bottomrule
    \end{tabular}
\end{table}

% \partitle{Passive Transfer Inference Attack}
% Given the victim knowledge graph holder $\mathcal{G}_v$, the adversary is a client. Adversary can observe the difference between the entity embedding matrix uploaded and downloaded to get the entities overlapping with other participants and the corresponding entity embedding matrix, including the entities overlapping $\mathcal{G}_v$ and the adversary. The adversary transfers the local relation embedding matrix to missing relation embedding matrix, and then infers the triple associated with the overlapping entity.

% \partitle{Active Transfer Inference Attack}
% Given the victim knowledge graph holder $\mathcal{G}_v$, we enhance the adversary's ability to infer the triples of $\mathcal{G}_v$ more accurately.
% Compared with passive attack, the adversary of active attack can not only observe client's information, but also change the entity embedding of the client.

% \partitle{Relation Inference Attack}
% Given the victim knowledge graph holder $\mathcal{G}_v$, the adversary is a malicious server with the victim model's entity set $\mathcal{E}_v$ and the entity embedding matrix $\bf{E}_v$ uploaded by the victim model.
% Therefore, relation attack can extend the inference scope to all triples of $\mathcal{G}_v$ compared to the limited inference scope of transfer attacks.

\subsection{Passive Transfer Inference Attack}
We first propose passive transfer inference attack, assume the adversary is a client of federated learning.

\partitle{Getting Overlapping Entities and Entity Embeddings}
In each round of training, the FKGE client will upload an entity embedding matrix to the server. And the server aggregates entity embedding matrix from all participants.
However, the aggregation strategy leads to that if an entity only appears in one certain knowledge graph, the corresponding embedding of the entity will not change.
Using this strategy, the adversary can compare the uploaded and downloaded entity embedding matrices to know which entities are overlapping.

\partitle{Transferring Relation Embeddings}
If the adversary wants to infer the triple of the victim knowledge graph $\mathcal{G}_v$ from the overlapping entity embedding matrix, he needs to use the score function, which is used to quantify the plausibility of a triple.
We transfer the adversary's local relation embeddings to complement the attack model's embedding matrix.
Intuitively, after federated training, local relation embeddings contain relation information of victim knowledge graph.

\partitle{Membership Inference}
Given a candidate triple $(h,r,t)$, our inferring is defined as follows.
\begin{equation} \nonumber
    \mathcal{A}_{pt}((h,r,t)) = 
    \begin{cases}
    1, f_r(\bf{h_1},\bf{t_1}) / \it f_r(\bf{h_2},\bf{t_2}) \geq \tau_{\it pt} \\
    0, f_r(\bf{h_1},\bf{t_1}) / \it f_r(\bf{h_2},\bf{t_2}) < \tau_{\it pt}
    \end{cases}
\end{equation}
where $\bf{h_1},\bf{t_1}$ are corresponding embeddings of $h, t$ in attack model's embedding matrix , $\bf{h_2},\bf{t_2}$ are corresponding embeddings of $h, t$ in adversary's local embeddings and $\tau_{pt}$ is tunable decision threshold in passive transfer inference attack. $\mathcal{A}((h,r,t))$ denotes the adversary's prediction on the sample $(h,r,t)$.

\subsection{Active Transfer Inference Attack}
Active transfer inference attack is based on passive transfer inference attack, adding the adversary's capability to modify the embedding.
Given a candidate triple $(h,r,t)$, the adversary reverses the entity embeddings for the entity embedding matrix uploaded in round $i$.
After $j$ rounds, the adversary compares the candidate triple scores in rounds $i$ and $i+j$ to infer whether it is a member of the victim knowledge graph.

\partitle{Reversing Entity Embeddings}
For triple $(h,r,t)$, we reverse its tail entity embedding, which will result in a larger score for this triple. At this point we record the triple score $s_1$.
Since the purpose of knowledge embedding training algorithm is to shrink the positive triple score, after $j$ rounds of training, a positive triple score will be transformed from an unreasonable $s_1$ to a smaller score.

\partitle{Membership Inference}
We record the $(h,r,t)$ score $s_2$ after $j$ rounds of training, and inferring is defined as follows.
\begin{equation} \nonumber
    \mathcal{A}_{at}((h,r,t)) = 
    \begin{cases}
    1, s_1 / s_2 \geq \tau_{at} \\
    0, s_1 / s_2 < \tau_{at}
    \end{cases}
\end{equation}
where $\tau_{at}$ is tunable decision threshold in active transfer inference attack.

\subsection{Relation Inference Attack}
Relation inference attack is our proposed server-based attack. In this attack, the adversary infers the relation membership, and then infers the complete triple membership.

\partitle{Calculating Inter-entity Embeddings}
At round $i$, the malicious server receives the full entity embedding matrix $\bf{E}_v$ of the victim KGE model. 
Adversary uses representations form of entities and relations (e.g., TransE \cite{DBLP:conf/nips/BordesUGWY13} representation form is $\bf{r = t - h}$) defined by various knowledge embedding algorithms to calculate the relation embeddings that may exist between each pair of entities.
The calculation method is as follows.
\begin{equation} \nonumber
\begin{split}
    &\bf{R} = \left\{\bf{r}_{\it i}\right\}_{i=1}^{n_v^2-n_v}, \\
    &\bf{r}_{\it i} = f_{e-r}(\bf{e}_{\it j}, \bf{e}_{\it k}), 0 \leq \it j < \it k < n_v
\end{split}
\end{equation}
where $n_v$ is the number of entities in the victim client and $f_{e-r}$ is the representation form of entities and relations.

Note that if the representation form of entities and relations cannot be converted to each other spatially, we will use $\bf{r = h - t}$ representations.

\partitle{Clustering Embeddings}
Clustering is to select out positive relation embeddings which tend to be more concentrated and closer to the center point in embedding space.
Adversary selects $\hat{m}$ embeddings according to the distance of the candidate embeddings from the cluster center, where $\hat{m}$ is a variable parameter representing the adversary's expectation of the number of relations.

\partitle{Membership Inference}
Given a candidate triple $(h,r,t)$, after the clustering embedding step, we get its connection $\left\{(h,x,t) | x\in\left\{0,1\right\}\right\}$.
With the help of auxiliary dataset $\mathcal{D}_{aux}$, the adversary is able to know the exact properties of connections.
In concretely, though two entities have the same label in knowledge graph, they represent two types of entities. However, if two relations have the same label, it means that these two relations represent the same relation type.
When adversary knows the exact properties of the connections, he can infer whether $(h,r,t)$ is a member of $\mathcal{G}_v$.


==> related_work.tex <==
\section{Related Work} \label{sec: related work}
\vspace{-0.5em}
\partitle{Membership Inference Attack}
Membership inference attack (MIA) aims to infer whether a data record has been used to train a machine learning model or not.
After Shokri et al. \cite{DBLP:conf/sp/ShokriSSS17}'s first MIA, extensive works have achieved successful attacks against various data domains, e.g., on image datasets \cite{DBLP:conf/nips/ZhuLH19, DBLP:conf/nips/GeipingBD020}, language datasets \cite{DBLP:journals/popets/HayesMDC19, DBLP:conf/ccs/SongR20}, or graph-structured datasets \cite{DBLP:conf/uss/HeJ0G021, DBLP:conf/sp/0011L0022, DBLP:journals/corr/abs-2110-02631}.
% Shokri et al. \cite{DBLP:conf/sp/ShokriSSS17} propose the first membership inference attacks against machine learning models.
% Salem et al. \cite{DBLP:conf/ndss/Salem0HBF019} propose a low-cost attack model via relaxing assumptions on the adversary.
% Nasr et al. \cite{DBLP:conf/sp/NasrSH19} extend membership inference attack to federated learning models by obtaining gradient updates.
% Hayes et al. \cite{DBLP:journals/popets/HayesMDC19} show that the adversary can infer whether a certain word in a participant's data by observing the non-zero gradients of the embedding layer in federated learning models.
In particular, Nasr et al. \cite{DBLP:conf/sp/NasrSH19} and Hayes et al. \cite{DBLP:journals/popets/HayesMDC19} propose MIAs on federated learning models by obtaining gradients updates.
MIAs against centralized graph neural networks \cite{DBLP:conf/uss/HeJ0G021, DBLP:conf/sp/0011L0022} or knowledge graphs \cite{DBLP:journals/corr/abs-2104-08273} reveals that graph-structured data is also at risk of privacy leakage.


% and most membership inference attacks against graph neural networks (GNN) exploit the similarity of node embeddings or the influence between nodes.
% He et al. \cite{DBLP:conf/uss/HeJ0G021} believe that the embeddings of adjacent nodes have a shorter distance.
% Wu et al. \cite{DBLP:conf/sp/0011L0022} re-identify private edges by calculating the influence between the nodes after adding a small perturbation.
% However, due to the rich properties of knowledge graph relationships, previous MIAs against GNN are hard to work.
 
% According to adversary's knowledge, membership inference attacks are divided into black-box attacks and white-box attacks.
% Attacks against federated learning are normally white-box attacks (capable of acquiring the structure of the target model, training parameters, and intermediate training updates).
% But in FKGE, adversary has no ability to access every training updates, making our attacks are more challenging than traditional white-box attacks on centralized learning.
% Different from the attack model of Wang et al. \cite{DBLP:journals/corr/abs-2104-08273} against the centralized knowledge embedding model, we conduct membership inference attacks on the knowledge embedding model in the federated learning.
% In our work, we observe and modify the gradient from target model. In addition, we introduce novel transfer-attacks and relation-attacks.
\vspace{-0.5em}

\partitle{Federated KGE and Privacy Protection}
% Knowledge graph embedding (KGE) is proposed to handle the difficulties in knowledge-based inferences and downstream applications \cite{DBLP:series/ssw/BianchiRCPM20, DBLP:journals/pieee/Nickel0TG16, DBLP:journals/tkde/WangMWG17} caused by the symbolic nature of knowledge graph.
% KGE models can be roughly divided into two categories: translational distance models, where a head embedding is translated to a tail embedding by a relation embedding, and bilinear models, where head and tail embeddings are combined by a bilinear matrix to measure the plausibility of a fact.
% The first translational distance models is TransE \cite{DBLP:conf/nips/BordesUGWY13}, which is extended by TransH \cite{DBLP:conf/aaai/WangZFC14}, TransR \cite{DBLP:conf/aaai/LinLSLZ15} and TransD \cite{DBLP:conf/acl/JiHXL015} for various scenarios.
% RotateE \cite{DBLP:conf/iclr/SunDNT19} replaces translation with rotation by introducing complex space to improve the ability of pattern modeling.
% RESCAL \cite{DBLP:conf/icml/NickelTK11} is the first bilinear KGE model, and DisMult \cite{DBLP:journals/corr/YangYHGD14a} restricts relation matrices in RESCAL as diagonal matrices.
% ComplEx \cite{DBLP:conf/icml/TrouillonWRGB16} further extends DisMult into complex space for properties like rotation and inversion.
% While most existing KGE models focus on a single knowledge graph, 
FedE \cite{DBLP:conf/jist/ChenZYJC21} is proposed as the first federated KGE framework, which aggregates locally computed updates of entity embeddings to train a global model. 
FedR \cite{DBLP:journals/corr/abs-2203-09553} aggregate relation embeddings instead of entity embeddings.
% Note that some other works also focus on distributed or decentralized KGE training \cite{DBLP:conf/dasfaa/DongWCLY20, DBLP:conf/edbt/Sheikh0GR22, DBLP:journals/corr/abs-2202-09512}, but they aim to distribute computation load for large-scale graphs, which is out of our scope in this paper, rather than protect the privacy of training data.
Although the training data is preserved locally in these federated frameworks, the transferred gradient updates may potentially encode fine details of at least some of the training data \cite{DBLP:conf/ccs/AbadiCGMMT016, DBLP:journals/fgcs/MothukuriPPHDS21} and can be leveraged to compromise the privacy of the training data \cite{DBLP:conf/uss/CarliniTWJHLRBS21, DBLP:journals/tsc/TruexLGYW21, DBLP:conf/sp/NasrSH19}.
DP has been investigated for KGE privacy protection.
Han et al. \cite{DBLP:journals/ws/HanDGCB22} propose a DPSGD-based DP KGE algorithm for a single KG in the centralized learning. Peng et al. \cite{DBLP:conf/cikm/PengLSZ021} propose a PATE-GAN-based DP KGE algorithm for multiple KGs in the decentralized learning with the off-the-shelf PATE-GAN technique \cite{DBLP:conf/iclr/JordonYS19a}. However, both works are not rigorous enough in DP analysis, which makes their DP guarantees hold only for part of the algorithms as detailed in Appendix \ref{appendix: inaccurate DP}.

% Although they also attempt to only perturb the active gradient elements binding to the sampled entities, they fail to conduct the selection in a differentially private manner. As a result, the overall DP guarantee is not satisfied as believed by the paper, because without DP perturbation the positions of the updated entities precisely tell which entities are in the training dataset and selected for update during iterations.
% attacker can easily infer which entities are included in the training dataset by observing which embeddings are updated.
% The authors notice that only a subset of all the embeddings are updated in each iteration and propose to only add noise to those embeddings which are involved in the current iteration (can be seen in Section 3.4 in the paper \cite{DBLP:journals/ws/HanDGCB22}). 
% We have to point out that this trick does not satisfy the definition of DP. 
% An intuitive explanation is that the attacker can determine which entities are included in the training dataset based on which embeddings are updated.

% Unlike traditional PATE-GAN usage where it feeds the generator with random inputs, \cite{DBLP:conf/cikm/PengLSZ021} feeds the generator with embeddings extracted from training KGs that should have been protected with DP. 
% As a reulst, the generated adversarial examples are transferred without any protection to the discriminators at another untrusted party(can be seen in Figure 3 and Algorithm 2 in the paper \cite{DBLP:conf/cikm/PengLSZ021}), thus FKGE is not a rigorous differential private algorithm. 
% As can be seen from the above discussion, a rigorous differentially private KGE algorithm under the federated setting still remains to be explored.


==> unused.tex <==
\partitle{Private Selection}
The private selection steps consist of two stages: Report-Noisy-Max and Propose-Test-Release. 
The exponential mechanism we use at the first stage is a Gumbel noise style implementation \cite{DBLP:conf/nips/DurfeeR19} which is analyzed with RDP via a ``Bounded Range'' property for tighter bound under composition. 
We adopt a PTR variant with Gaussian noise \cite{DBLP:conf/aistats/0005W22} for the second stage.
Since there is a probability bounded by $\delta_t$ that the test in PTR may fail, the algorithm satisfies an approximated RDP.
The privacy guarantee of private selection without subsampling is shown in lemma \ref{lemma:private selection} by using the RDP composition theorem in lemma \ref{lemma: rdp composition}.
\begin{lemma}\label{lemma:private selection}
    The private selection in Algorithm \ref{alg: private selection} without subsampling satisfies $\delta_t$-approximated-$(\alpha, (\frac{\alpha}{8\sigma_r^2}+\frac{\alpha}{2\sigma_p^2}))$-RDP.
\end{lemma}

The input of Algorithm \ref{alg: private selection} is produced with triples subsampled from the original dataset(line 11 in Algorithm \ref{alg: dpsgd with private selection}), thus the privacy guarantee can be amplified through subsampling.
By using the privacy amplification theorem for RDP with subsampled mechanism \cite{DBLP:conf/aistats/WangBK19}, we have a tighter privacy guarantee in lemma \ref{lemma: subsampled private selection}.

\begin{lemma}\label{lemma: subsampled private selection}
    The private selection in Algorithm \ref{alg: private selection} with subsampling rate $q$ satisfies $\delta_t$-approximated-$(\alpha, \epsilon'(\alpha))$-RDP, where
    \begin{align}
        \nonumber \epsilon'(\alpha)=&\frac{1}{\alpha-1}\log(1+p^2\tbinom{\alpha}{2}\min\{4(e^{\epsilon(2)}-1),\\ 
        \nonumber &\qquad\qquad\qquad\ \ \, e^{\epsilon(2)}\min\{2, (e^{\epsilon(\infty)}-1)^2\}\}\\
        \nonumber &+\sum_{j=3}^\alpha q^j\tbinom{\alpha}{j}e^{(j-1)\epsilon(j)}\min\{2,(e^{\epsilon(\infty)}-1)^j\}),\\
        \nonumber and\qquad&\\
        \nonumber \epsilon(\alpha)=&\frac{\alpha}{8\sigma_r^2}+\frac{\alpha}{2\sigma_p^2}.
    \end{align}
\end{lemma}

With the above components, we propose the privacy guarantee of each iteration in our differentially private KGE training as shown in lemma \ref{theorem: iteration}
\begin{theorem}\label{theorem: iteration}
    Each iteration in Algorithm \ref{alg: dpsgd with private selection} satisfies $\delta_t$-approximated-$(\alpha, \frac{2q^2\alpha}{\sigma}+\epsilon'(\alpha))$-RDP and $(\frac{2q^2\alpha}{\sigma}+\epsilon'(\alpha)+\frac{\log(1/\delta)}{\alpha-1}, \delta+\delta_t)$-DP, where $\alpha$ meets the constrain in lemma \ref{lemma:dpsgd} and $\epsilon'(\alpha)$ is the same as in lemma \ref{lemma: subsampled private selection}.
\end{theorem}
